WoVoGen: World Volume-aware Diffusion for Controllable Multi-camera Driving Scene Generation

Generating multi-camera street-view videos is critical for augmenting autonomous driving datasets, addressing the urgent demand for extensive and varied data. Due to the limitations in diversity and challenges in handling lighting conditions, traditional rendering-based methods are increasingly being supplanted by diffusion-based methods. However, a significant challenge in diffusion-based methods is ensuring that the generated sensor data preserve both intra-world consistency and inter-sensor coherence. To address these challenges, we combine an additional explicit world volume and propose the World Volume-aware Multi-camera Driving Scene Generator (WoVoGen). This system is specifically designed to leverage 4D world volume as a foundational element for video generation. Our model operates in two distinct phases: (i) envisioning the future 4D temporal world volume based on vehicle control sequences, and (ii) generating multi-camera videos, informed by this envisioned 4D temporal world volume and sensor interconnectivity. The incorporation of the 4D world volume empowers WoVoGen not only to generate high-quality street-view videos in response to vehicle control inputs but also to facilitate scene editing tasks.

==> figures/editing.tex <==
\begin{figure*}[h]  
\centering  
\includegraphics[width=\linewidth]{images/control.png} 
\caption{\textbf{Enhanced generation control and editing capabilities are integral aspects of the proposed \abb{}}. In comparison to related works, \abb{} exhibits noteworthy features:(a) Accepts location-based text prompts, facilitating the generation of localized images.
(b) Enables arbitrary editing of world volume grids, ensuring the generation of geometrically consistent images.
(c) Demonstrates the ability to modify camera parameters, allowing for the generation of ego car observations from diverse perspectives.}
\label{fig:cig}  
\end{figure*} 

==> figures/sub_architecture.tex <==
\begin{figure}[t]
\centering  
\includegraphics[width=0.6\linewidth]{images/sub_pipe.pdf} 
\caption{
{\bf (a)}: an action attention block enhances the model by incorporating essential action information.
{\bf (b)}: a guidance attention block integrates the CLIP feature of a specific object into the latent representation, further refining the model's capabilities.
}
\label{fig:sub_architecture}  
\end{figure} 

==> figures/supply/object_guidance_ablation.tex <==
\begin{figure*}[h]  
\centering  
\includegraphics[width=\linewidth]{images/supply/object_ablation.pdf} 
\caption{\textbf{Qualitative ablation study on object guidance.} The incorporation of object guidance significantly improves the alignment of the generated image's object with the target image.} 
\label{fig:obg_ab}  
\vspace{-0.2cm}
\end{figure*}

==> tables/obj_guid_and_kpm.tex <==
\renewcommand\arraystretch{1.2} 
\begin{table}[htb] 
    % \scriptsize
	 \noindent
 \begin{minipage}{0.5\textwidth}
 \centering 
 
  \setlength{\tabcolsep}{1mm}
     \caption{Quantitative comparison of image generation quality on the nuScenes validation set with and without object guidance.}
 
	\begin{tabular}{cc|c} 
	\hline

 \hline
    \rowcolor{gray!20}
    World Volume & Object Guidance & \textbf{FID$\downarrow$} \\
	\hline

    $\times$ & $\checkmark$ & 28.6 \\ 
    $\checkmark$ & $\times$ & 27.8  \\ 
     $\checkmark$ & $\checkmark$ & \textbf{27.6}\\
    
	\hline

 \hline
	\end{tabular}
         
	\label{tab:obg_ab}
 \end{minipage}
\hspace{2em}
  \begin{minipage}{0.4\textwidth}
  \setlength{\tabcolsep}{1mm}
  \centering 
     \caption{Quantitative results of .}
 
	\begin{tabular}{c|c} 
	\hline

 \hline
    \rowcolor{gray!20}
    Consistency & KPM \\
	\hline

    Multi-view &  90.0 \\ 
    Temporal& 80.2 \\ 
    
	\hline

 \hline
	\end{tabular}
         
	\label{tab:obg_ab}
 \end{minipage}
 
\end{table}
